Introduction to Rank-polymorphic Programming in Remora (Draft)

Remora is a higher-order, rank-polymorphic array-processing programming language, in the same general class of languages as APL and J. It is intended for writing programs to be executed on parallel hardware. We provide an example-driven introduction to the language, and its general computational model, originally developed by Iverson for APL. We begin with Dynamic Remora, a variant of the language with a dynamic type system (as in Scheme or Lisp), to introduce the fundamental computational mechanisms of the language, then shift to Explicitly Typed Remora, a variant of the language with a static, dependent type system that permits the shape of the arrays being computed to be captured at compile time. This article can be considered an introduction to the general topic of the rank-polymorphic array-processing computational model, above and beyond the specific details of the Remora language. We do not address the details of type inference in Remora, that is, the assignment of explicit types to programs written without such annotations; this is ongoing research.

==> decls.tex <==
% Macros used in the paper					% -*- latex -*-

\makeatletter

\newcommand{\ie}{\mbox{\emph{i.e.}}}
\newcommand{\Ie}{\mbox{\emph{I.e.}}}
\newcommand{\eg}{\mbox{\emph{e.g.}}}
\newcommand{\Eg}{\mbox{\emph{E.g.}}}
\newcommand{\etc}{\emph{etc.}}
\newcommand{\nb}{\mbox{\emph{n.b.}}}
\newcommand{\Nb}{\mbox{\emph{N.b.}}}

\newcommand{\sequence}[1]{#1 \, \ldots \,}
\newcommand{\llb}{\left\llbracket}
\newcommand{\rrb}{\right\rrbracket}

\let\oldl\l %Save the old \l on \oldl
\newcommand{\cl}{\llap{$\lambda$\hskip-.65em}\phantom{ss}}
%% JFP-friendly versions of \lambda-in-code macros
\renewcommand{\l}[1]{\cl(#1)}
%% Non-JFP versions of \lambda-in-code macros
% \renewcommand{\l}[1]{\ \llap{$\lambda$\hskip-.5em}\ (#1)}

%% What you frequently want when you say \tt:
\def\ttt{\ttfamily\upshape\mdseries\catcode``=13}%\frenchspacing\@noligs

%% Centered version of alltt environment
\newenvironment{centertt}{%
  \par\medskip
  \centering
  \varwidth{\linewidth}%
  \alltt
}{%
  \endalltt
  \endvarwidth
  \vspace{-5pt}
  \par
}

\newcommand{\itum}[1]{\item{\bf #1}\\*}

% Works in math mode; all special chars remain special; cheaper than \cd.
% Will not be correct size in super and subscripts, though.
\newcommand{\ex}[1]{\mbox{\ttt{#1}}}

\newenvironment{inset}
 {\bgroup\parskip=1ex plus 1ex\begin{list}{}%
        {\topsep=0pt\rightmargin\leftmargin}%
        \item[]}%
 {\end{list}\leavevmode\egroup\global\@ignoretrue}

\newenvironment{tightinset}
 {\bgroup\parskip=0pt\begin{list}{}%
        {\topsep=0pt\rightmargin\leftmargin}%
        \item[]}%
 {\end{list}\leavevmode\egroup\ignorespaces}

\newenvironment{leftinset}
 {\bgroup\parskip=1ex plus 1ex\begin{list}{}%
        {\topsep=0pt}%
        \item[]}%
 {\end{list}\leavevmode\egroup\global\@ignoretrue}

% For typesetting interactive examples.
\newcommand{\result}[1]{\textsl{#1}}

% For multiletter vars in math mode:
\renewcommand{\v}[1]{\ensuremath{\mathit{#1}}} % \frenchspacing?
\newcommand{\vi}[2]{\ensuremath{\mathit{#1}_{#2}}}

% Remora type constructors
\newcommand{\tu}{\ensuremath{\rightarrow}}
\newcommand{\ft}[2]{(\tu\ (#1) #2)}
\newcommand{\faty}[2]{(\ensuremath{\forall} (#1) {#2})}
\newcommand{\pity}[2]{(\ensuremath{\Pi} (#1) {#2})}
\newcommand{\boxtype}[1]{\ensuremath{\Sigma} (#1)}

\makeatother

